Stable Unlearnable Example: Enhancing the Robustness of Unlearnable Examples via Stable Error-Minimizing Noise

The open source of large amounts of image data promotes the development of deep learning techniques. Along with this comes the privacy risk of these open-source image datasets being exploited by unauthorized third parties to train deep learning models for commercial or illegal purposes. To avoid the abuse of public data, a poisoning-based technique, the unlearnable example, is proposed to significantly degrade the generalization performance of models by adding a kind of imperceptible noise to the data. To further enhance its robustness against adversarial training, existing works leverage iterative adversarial training on both the defensive noise and the surrogate model. However, it still remains unknown whether the robustness of unlearnable examples primarily comes from the effect of enhancement in the surrogate model or the defensive noise. Observing that simply removing the adversarial noise on the training process of the defensive noise can improve the performance of robust unlearnable examples, we identify that solely the surrogate model's robustness contributes to the performance. Furthermore, we found a negative correlation exists between the robustness of defensive noise and the protection performance, indicating defensive noise's instability issue. Motivated by this, to further boost the robust unlearnable example, we introduce stable error-minimizing noise (SEM), which trains the defensive noise against random perturbation instead of the time-consuming adversarial perturbation to improve the stability of defensive noise. Through extensive experiments, we demonstrate that SEM achieves a new state-of-the-art performance on CIFAR-10, CIFAR-100, and ImageNet Subset in terms of both effectiveness and efficiency. The code is available at https://github.com/liuyixin-louis/Stable-Unlearnable-Example.

==> lib/common_used.tex <==

\usepackage{booktabs}
\usepackage{csquotes}
\usepackage{amsmath}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{amssymb}
\usepackage{lipsum}
\usepackage{multirow}
\usepackage{graphicx}
% \usepackage{wrapfig}
% \usepackage{}
\usepackage{amsmath,amsfonts,bm}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{enumitem}

\usepackage{hyperref}
\usepackage{url}
\usepackage{graphicx}
% \usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{subcaption}


% Expectation symbol
\DeclareMathOperator*{\E}{\mathbb{E}}
\newcommand{\BK}[1]{\textcolor{red}{BK: #1}}
\newcommand{\rwd}{\text{rewinding}\xspace}
\newcommand{\RWD}{\text{Rewinding}\xspace}
\newcommand{\init}{\text{initialization}\xspace}
\newcommand{\INIT}{\text{Initialization}\xspace}
\newcommand{\posthoc}{\text{traditional}\xspace}
\newcommand{\POSTHOC}{\text{Traditional}\xspace}
\newcommand{\cnet}{\texttt{CARD}\xspace}
\newcommand{\cnets}{\texttt{CARDs}\xspace}
\newcommand{\chand}{\texttt{CARD-Hand}\xspace}
\newcommand{\cdeck}{\texttt{CARD-Deck}\xspace}
\newcommand{\cdecks}{\texttt{CARD-Decks}\xspace}
\newcommand{\RMV}[1]{\textcolor{blue}{RMV: #1}}
\newcommand{\BB}[1]{\textcolor{green!90}{BB: #1}}
% \newcommand{\ie}{\textit{i}.\textit{e}.}
% \newcommand{\eg}{\textit{e}.\textit{g}.}
\newcommand{\stdv}[1]{\scriptsize$\pm$#1}

\def \ind {\mathds{1}}
\def \cD {\mathcal{D}}
\def \cA {\mathcal{A}}
\def \cF {\mathcal{F}}
\def \cR {\mathcal{R}}
\def \cL {\mathcal{L}}
\def \bbR {\mathbb{R}}
\def \bbE {\mathbb{E}}

\def \vx {\bm{x}}
\def \vp {\bm{p}}
\def \vg {\bm{g}}
\def \vw {\bm{w}}

\def \hyp {\mathrm{hyp}}
\def \adv {\mathrm{adv}}
\def \sta {\mathrm{sta}}
\def \nat {\mathrm{nat}}
\def \linf {\ell_{\infty}}

\def\todo{\textcolor{blue}}

\usepackage{algpseudocode}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\rightt}{$\checkmark$}
\newcommand{\wrongg}{$\times$}
% \newcommand{\wronggg}{$\times$}

\usepackage{appendix}

% \usepackage{subfigure}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> lib/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tab/ablation.tex <==

\begin{table}[htbp]
\renewcommand{\arraystretch}{0.7}
\centering
\caption{The Ablation study of the proposed random perturbation term on CIFAR-10. We denote the training process as $\mathcal{T}$, and the final regeneration process as $\mathcal{G}$. We study the effectiveness of random perturbation in these two phases by removing them respectively.}
\label{tab: ablation}
\scriptsize
\begin{tabular}{cccccc} 
    \toprule
    \multicolumn{2}{c}{Ablation Setting}            & \multicolumn{2}{c}{$\rho_u=8/255$} & \multicolumn{2}{c}{$\rho_u=16/255$}  \\
    \cmidrule(l){1-6}
    $\mathcal{T}$          & $\mathcal{G}$          & $\rho_a=2/255$ & $4/255$           & $\rho_a=4/255$ & $8/255$             \\
    \midrule
    $\checkmark$ & $\checkmark$ & \textbf{20.20} & \textbf{30.48} & \textbf{15.20} & \textbf{24.22} \\
    $\times$ & $\checkmark$ & 18.41 & 29.82 & 13.25 & 27.25 \\
    $\checkmark$ & $\times$ & 19.93 & 32.44 & 16.01 & 25.86 \\
    $\times$ & $\times$ & 18.01 & 31.24 & 14.31 & 26.27 \\
    \bottomrule
\end{tabular}

    

\end{table}


==> tab/adv_setting.tex <==

\begin{table}[htbp]
	\centering
	\caption{
	The settings of PGD for the noise generations of different baseline methods. $\rho_u$ denotes the defensive perturbation radius of different types of noise, while $\rho_a$ denotes the adversarial perturbation radius of the robust error-minimizing noise.
	}
	\label{tab: pgd_params}
	\scriptsize
	\begin{tabular}{cccccc} 
\toprule
Datasets                                                                       & Noise Type     & $\alpha_d$   & $K_d$ & $\alpha_a$ & $K_a$  \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR-10 \\ CIFAR-100\end{tabular}} & EM             & $\rho_u/5$   & $10$  & -          & -      \\
                                                                               & TAP            & $\rho_u/125$ & $250$ & -          & -      \\
                                            
                                                                               & REM \& SEM(Ours) & $\rho_u/5$   & $10$  & $\rho_a/5$ & $10$   \\ 
\midrule
\multirow{3}{*}{ImageNet Subset}                                               & EM             & $\rho_u/5$   & $7$   & -          & -      \\
                                                                               & TAP            & $\rho_u/50$  & $100$ & -          & -      \\                                                                               & REM \& SEM(Ours) & $\rho_u/4$   & $7$   & $\rho_a/5$ & $10$   \\
\bottomrule
\end{tabular}
\label{tab:adv}
\end{table}


==> tab/combination.tex <==

\begin{table*}[!thbp]
    \centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lllllll} 
\toprule
\multirow{2}{*}{No.~~} & \multirow{2}{*}{Test Acc} & \multicolumn{2}{c}{$\delta^{u*}$}                                   & \multicolumn{2}{c}{$\theta^*$}                                      & \multicolumn{1}{c}{\multirow{2}{*}{Note}}                                                \\ 
\cmidrule(l){3-6}
                       &                           & \multicolumn{1}{c}{$\delta^{r}$} & \multicolumn{1}{c}{$\delta^{a}$} & \multicolumn{1}{c}{$\delta^{r}$} & \multicolumn{1}{c}{$\delta^{a}$} & \multicolumn{1}{c}{}                                                                     \\ 
\midrule
\#1                    &   0.47                        & \multicolumn{1}{c}{$\surd$}      & \multicolumn{1}{c}{$\surd$}      & \multicolumn{1}{c}{$\surd$}      & \multicolumn{1}{c}{$\surd$}      & \multicolumn{1}{c}{All present}                                                          \\
\#2                    &     0.8932                  & $\surd$                          & $\surd$                          & $\surd$                          &                                  & Random noise and adversarial noise in $\delta^u*$, only random noise in $\theta^*$       \\
\#3                    &       0.4417                    & $\surd$                          & $\surd$                          &                                  & $\surd$                          & Random noise and adversarial noise in $\delta^u*$, only adversarial noise in $\theta^*$  \\
\#4                    &      0.8869                     & $\surd$                          & $\surd$                          &                                  &                                  & Only random noise and adversarial noise in $\delta^u*$                                   \\
\#5                    &      0.359633                     & $\surd$                          &                                  & $\surd$                          & $\surd$                          & Random noise in both $\delta^u*$ and $\theta^*$, only adversarial noise in $\theta^*$    \\
\#6                    & 0.894567                  & $\surd$                          &                                  & $\surd$                          &                                  & Only random noise in both $\delta^u*$ and $\theta^*$                                     \\
\#7                    & \textbf{0.300267}         & $\surd$                          &                                  &                                  & $\surd$                          & Random noise in $\delta^u*$, adversarial noise in $\theta^*$ \textbf{SEM-v1}                            \\
\#8                    & 0.892167                  & $\surd$                          &                                  &                                  &                                  & Only random noise in $\delta^u*$                                                   \\
\#9                    &    0.4435                      &                                  & $\surd$                          & $\surd$                          & $\surd$                          & Adversarial noise in both $\delta^u*$ and $\theta^*$, only random noise in $\theta^*$    \\
\#10                   & 0.892733                  &                                  & $\surd$                          & $\surd$                          &                                  & Only adversarial noise in $\delta^u*$, random noise in $\theta^*$                        \\
\#11                   & 0.467200                  &                                  & $\surd$                          &                                  & $\surd$                          & Adversarial noise in both $\delta^u*$ and $\theta^*$ \textbf{REM}                                 \\
\#12                   & 0.882800                  &                                  & $\surd$                          &                                  &                                  & Only adversarial noise in $\delta^u*$                                                    \\
\#13                   &      0.349433                     &                                  &                                  & $\surd$                          & $\surd$                          & Both noises in $\theta^*$                                                                \\
\#14                   & 0.890733                  &                                  &                                  & $\surd$                          &                                  & Only random noise in $\theta^*$                                                          \\
\#15                   & 0.379067                  &                                  &                                  &                                  & $\surd$                          & Only adversarial noise in $\theta^*$                                                     \\
\#16                   & 0.891533                  &                                  &                                  &                                  &                                  & No noise in both $\delta^u*$ and $\theta^*$ \textbf{EM}                                            \\
\bottomrule
\end{tabular}
}
    \caption{All the case. The lower the test acc indicates better performance. \rtodo{Observations: 1. with adv noise tuning on in theta training, adding randomness when during neither noise nor theta improve performance (\#7 and \# 13) and adding it to the noise seem to be better; 2. theta need adv noise while delta needs random noise to train. } I think the story can be formulated into like when training the noise, its ability to defend against random perturbation is more important. 
    So it seems adding adv noise to delta training is hurtful. }
    \label{tab: all case}
\end{table*}

==> tab/diff_perc.tex <==
\begin{table*}[t]
    \renewcommand{\arraystretch}{0.7}
    \centering
    \caption{Test accuracy (\%) on CIFAR-10 and CIFAR-100 with different protection percentages. We set the defensive perturbation radius $\rho_u$ as $8/255$. For REM and SEM, we set $\rho_a$ and $\rho_a$ as $4/255$. 
    }
    \label{tab:diff_perc_c10}
    \resizebox{.9\linewidth}{!}{
        \begin{tabular}{cccc|cc|cc|cc|cc|c} 
            \toprule
            \multirow{3}{*}{Dataset}    & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Adv. \\ Train. \\ $\rho_a$\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Noise \\ Type\end{tabular}} & \multicolumn{10}{c}{Data Protection Percentage}                                                                                                                                                                          \\ 
            \cmidrule{4-13}
                                        &                                                                                     &                                                                        & \multirow{2}{*}{0\%}   & \multicolumn{2}{c|}{20\%}               & \multicolumn{2}{c|}{40\%}               & \multicolumn{2}{c|}{60\%}               & \multicolumn{2}{c|}{80\%}               & \multirow{2}{*}{100\%}  \\
                                        &                                                                                     &                                                                        &                        & Mixed          & Clean                  & Mixed          & Clean                  & Mixed          & Clean                  & Mixed          & Clean                  &                         \\ 
            \midrule
            \multirow{12}{*}{CIFAR-10}  & \multirow{6}{*}{$2/255$}                                                            & EM                                                                     & \multirow{6}{*}{92.37} & 92.26          & \multirow{6}{*}{91.30} & 91.94          & \multirow{6}{*}{90.31} & 91.81          & \multirow{6}{*}{88.65} & 91.14          & \multirow{6}{*}{83.37} & 71.43                   \\
                                        &                                                                                     & TAP                                                                    &                        & \textbf{92.17} &                        & 91.62          &                        & 91.32          &                        & 91.48          &                        & 90.53                   \\
                                        &                                                                                     & NTGA                                                                   &                        & 92.41          &                        & 92.19          &                        & 92.23          &                        & 91.74          &                        & 85.13                   \\
                                        &                                                                                     & SC                                                                &&92.3&&	91.98&&90.17&&87.58&&	47.66   \\
                                        &                                                                                     & REM                                                                    &                        & 92.36          &                        & \textbf{90.22} &                        & 88.45          &                        & \textbf{82.98} &                        & 30.69                   \\
                                        &                                                                                     & SEM                                                                    &                        & 91.94 && 90.89 && 88.90 && 84.82 && \textbf{11.32}    \\ 
            \cmidrule{2-13}
                                        & \multirow{6}{*}{$4/255$}                                                            & EM                                                                     & \multirow{6}{*}{89.51} & 89.60          & \multirow{6}{*}{88.17} & 89.40          & \multirow{6}{*}{86.76} & 89.49          & \multirow{6}{*}{85.07} & 89.10          & \multirow{6}{*}{79.41} & 88.62                   \\
                                        &                                                                                     & TAP                                                                    &                        & \textbf{89.01} &                        & \textbf{88.66} &                        & 88.40          &                        & 88.04          &                        & 88.02                   \\
                                        &                                                                                     & NTGA                                                                   &                        & 89.56          &                        & 89.35          &                        & 89.22          &                        & 89.17          &                        & 88.96                   \\
                                        &                                                                                     & SC                                                        && 89.4&&	89.14&&	89.23&&	89.02&&	84.43        \\
                                        &                                                                                     & REM                                                                    &                        & 89.60          &                        & 89.34          &                        & 89.61          &                        & 88.09          &                        & 48.16                   \\
                                        &                                                                                     & SEM                                                                    &                        & 89.82 && 89.65 && 88.66 && 85.19 && \textbf{31.29}      \\ 
            \midrule
            \multirow{12}{*}{CIFAR-100} & \multirow{6}{*}{$2/255$}                                                            & EM                                                                     & \multirow{6}{*}{68.91} & 68.51          & \multirow{6}{*}{66.54} & 68.72          & \multirow{6}{*}{64.21} & 67.96          & \multirow{6}{*}{58.35} & 68.44          & \multirow{6}{*}{47.99} & 68.49                   \\
                                        &                                                                                     & TAP                                                                    &                        & \textbf{68.05} &                        & 67.83          &                        & 67.75          &                        & 67.27          &                        & 66.91                   \\
                                        &                                                                                     & NTGA                                                                   &                        & 68.52          &                        & 68.82          &                        & 68.36          &                        & 68.71          &                        & 66.53                   \\
                                        &                                                                                     & SC                                                                     &                        & 68.22 && 68.21 && 67.05 && 62.25 && 29.58 \\
                                        &                                                                                     & REM                                                                    &                        & 69.00          &                        & 68.20          &                        & \textbf{60.75} &                        & \textbf{52.33} &                        & 7.03                    \\
                                        &                                                                                     & SEM                                                                    &                        & 68.89 && 68.10 && 60.92 && 53.87 && \textbf{4.41}       \\ 
            \cmidrule{2-13}
                                        & \multirow{6}{*}{$4/255$}                                                            & EM                                                                     & \multirow{6}{*}{64.50} & 63.86          & \multirow{6}{*}{61.73} & 64.24          & \multirow{6}{*}{57.61} & 63.62          & \multirow{6}{*}{53.86} & 63.37          & \multirow{6}{*}{44.79} & 63.43                   \\
                                        &                                                                                     & TAP                                                                    &                        & \textbf{63.21} &                        & \textbf{63.01} &                        & \textbf{62.95} &                        & 62.90          &                        & 62.39                   \\
                                        &                                                                                     & NTGA                                                                   &                        & 63.48          &                        & 63.59          &                        & 63.64          &                        & \textbf{62.83} &                        & 62.44                   \\
                                        &                                                                                     & SC                                                                     &                        &   63.28 && 63.72 && 63.64 && 63.81 && 61.41 \\
                                        &                                                                                     & REM                                                                    &                        & 63.75          &                        & 63.99          &                        & 64.36          &                        & 63.05          &                        & 27.10                   \\
                                        &                                                                                     & SEM                                                                    &                        & 63.94 && 64.05 && 63.75 && 64.43 && \textbf{20.25}  \\
            \hline
            \end{tabular}
    }
    
    % \vspace{-3mm}
    \label{tab: diff_perc}
    \end{table*}



==> tab/diff_radius.tex <==
\begin{table*}[t]
%\small
\centering
\caption{Test accuracy (\%) of models trained on data protected by different defensive noises via adversarial training with different perturbation radii. The defensive perturbation radius $\rho_u$ is set as $8/255$ for every type of noise, while the adversarial perturbation radius $\rho_a$ of REM noise takes various values. $\Delta$ denotes the difference in test accuracy between the models trained on the data protected by SEM and REM, which indicates the data protection performance gain of SEM compared to the REM baseline. We specify that the higher the value of $\Delta$, the better the effectiveness of the protection. We denote \colortext{Maroon}{improvement ($\uparrow$)} and \colortext{ForestGreen}{reduction ($\downarrow$)} using different color. The same notation will be applied in the following tables. 
}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|ccccc|ccccc|ccccc} 
\toprule
Dataset$\rightarrow$     & \multicolumn{5}{c}{CIFAR-10}               & \multicolumn{5}{c}{CIFAR-100}         & \multicolumn{5}{c}{Tiny-ImageNet}    \\ 
\cmidrule(lr){1-1}\cmidrule(lr){2-6}\cmidrule(lr){7-11}\cmidrule(lr){12-16}
                           Method$\downarrow$ & $\rho_a$=0 & 1/255 & 2/255 & 3/255 & 4/255 & 0     & 1/255 & 2/255 & 3/255 & 4/255 & 0     & 1/255 & 2/255 & 3/255 & 4/255  \\ 
\midrule
Clean                       & 94.66      & 93.74 & 92.37 & 90.90 & 89.51 & 76.27 & 71.90 & 68.91 & 66.45 & 64.50 & 98.21 & 97.20 & 96.51 & 95.44 & 95.28  \\
TAP~\cite{fowl2021adversarial}                         & 22.51      & 92.16 & 90.53 & 89.55 & 88.02 & 13.75 & 70.03 & 66.91 & 64.30 & 62.39 & 58.54 & 97.80 & 96.62 & 97.50 & 98.00  \\
EM~\cite{huang2021unlearnable}                              & 13.20      & 22.08 & 71.43 & 87.71 & 88.62 & 1.60  & 71.47 & 68.49 & 65.66 & 63.43 & 69.12 & 52.50 & 55.51 & 56.74 & 54.57  \\
Shortcut~\cite{yuAvailabilityAttacksCreate2022}                    & 11.63      & 91.71 & 90.42 & 86.84 & 87.26 &\textbf{ 1.51}  & 70.62 & 67.95 & 65.81 & 63.30 & 49.25 & 97.20 & 96.51 & 95.44 & 95.28  \\
REM~\cite{fuRobustUnlearnableExamples2022}                         & 15.18      & \textbf{14.28} & 25.41 & 30.85 & 48.16 & 1.89  & 4.47  & 7.03  & 17.55 & 27.10 & 54.12 & \textbf{54.36} & 53.16 & 52.52 & 53.44  \\ \midrule
\textbf{SEM} & \textbf{10.68}      & 16.87 & \textbf{12.38} & \textbf{12.53} & \textbf{18.78} & 1.70  & \textbf{4.00 } & \textbf{3.00}  & \textbf{9.52}  & \textbf{20.08} & \textbf{46.50} & 54.51 & \textbf{52.45} & \textbf{51.12} & \textbf{51.79}  \\
$\Delta$ (\colortext{Maroon}{$\uparrow$}/\colortext{ForestGreen}{$\downarrow$}) & \gain{+4.50} & \reduc{-2.59} & \gain{+4.50} & \gain{+13.03} & \gain{+18.32} &\reduc{-0.19}&\gain{+0.47}&\gain{+4.03} &\gain{+8.03} &\gain{+7.02} &\gain{+7.62} &\reduc{-0.15} &\gain{+0.71}&\gain{+1.40}&\gain{+1.65}
\\

\bottomrule
\end{tabular}
}

\label{tab:diff_rad}
\end{table*}


==> tab/diff_random.tex <==
\begin{table}[!t]
\centering
\caption{Comparison of the effectiveness of different random noise distributions on CIFAR-10. The radius of random noise and adversarial noise is set as $4/255$, and the radius of defensive noise is set to $8/255$. 
}
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Distribution} & \multicolumn{3}{c}{Training} &  \multicolumn{2}{c}{Evaluation}\\
 & TrainAcc & TestAcc & TimeCost & TrainAcc & TestAcc \\
\midrule
\texttt{Beta} & 90.62 & 23.54 & 5.78 & 100 &\textbf{ 28.23} \\
\texttt{Uniform} & 94.53 & 27.17 & 5.84 & 100 & 30.26 \\
\texttt{Gaussian} & 98.44 & 33.11 & 5.83 & 100 & 37.31 \\
\bottomrule
\end{tabular}
}

\label{tab:diff_noise_time}
\end{table}


==> tab/diff_rates.tex <==

\begin{table*}[!htbp]
\centering
\caption{Test accuracy (\%) on CIFAR-10 and CIFAR-100 with different protection percentages. For EM, TAP, and Shortcut noises, the perturbation radius $\rho_u$ is set as $8/255$. For REM and SEM noise, the perturbation radii $\rho_u$ and $\rho_a$ are set as $8/255$ and $4/255$, respectively.
}
\label{tab:diff_perc_c10}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccl|cc|cc|cc|cc|c} 
\toprule
\multirow{3}{*}{Dataset}    & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Adv. \\ Train. \\ $\rho_a$\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Noise \\ Type\end{tabular}} & \multicolumn{10}{c}{Data Protection Percentage}                                                                                                                                                                                                                                                                          \\ 
\cmidrule{4-13}
                            &                                                                                     &                                                                        & \multirow{2}{*}{0\%}   & \multicolumn{2}{c|}{20\%}                          & \multicolumn{2}{c|}{40\%}                                   & \multicolumn{2}{c|}{60\%}                                   & \multicolumn{2}{c|}{80\%}                                                & \multirow{2}{*}{100\%}              \\
                            &                                                                                     &                                                                        &                        & Mixed                     & Clean                  & Mixed                              & Clean                  & Mixed                              & Clean                  & Mixed                                           & Clean                  &                                     \\ 
\midrule
\multirow{10}{*}{CIFAR-10}  & \multirow{5}{*}{$2/255$}                                                            & EM                                                                     & \multirow{5}{*}{92.37} & 92.26                     & \multirow{5}{*}{91.30} & 91.94                              & \multirow{5}{*}{90.31} & 91.81                              & \multirow{5}{*}{88.65} & 91.14                                           & \multirow{5}{*}{83.37} & 71.43                               \\
                            &                                                                                     & TAP                                                                    &                        & \textbf{92.17}            &                        & 91.62                              &                        & 91.32                              &                        & 91.48                                           &                        & 90.53                               \\
                            &                                                                                     & Shortcut                                                                   &                        & 92.41                     &                        & 92.19                              &                        & 92.23                              &                        & 91.74                                           &                        & 85.13                               \\
                            &                                                                                     & REM                                                                    &                        & 92.36                     &                        & \textbf{90.22}                     &                        & 88.45                              &                        & \textbf{82.98}                                  &                        & 30.69                               \\
                            &                                                                                     & SEM                                                                   &                        & 92.23                     &                        & 90.76                              &                        & \textbf{88.44}                     &                        & 83.28                                           &                        & \textbf{12.38}                      \\ 
\cmidrule{2-13}
                            & \multirow{5}{*}{$4/255$}                                                            & EM                                                                     & \multirow{5}{*}{89.51} & 89.60                     & \multirow{5}{*}{88.17} & 89.40                              & \multirow{5}{*}{86.76} & 89.49                              & \multirow{5}{*}{85.07} & 89.10                                           & \multirow{5}{*}{79.41} & 88.62                               \\
                            &                                                                                     & TAP                                                                    &                        & \textbf{89.01}            &                        & \textbf{88.66}                     &                        & 88.40                              &                        & 88.04                                           &                        & 88.02                               \\
                            &                                                                                     & Shortcut                                                                   &                        & 89.56                     &                        & 89.35                              &                        & 89.22                              &                        & 89.17                                           &                        & 88.96                               \\
                            &                                                                                     & REM                                                                    &                        & 89.60                     &                        & 89.34                              &                        & 89.61                              &                        & 88.09                                           &                        & 48.16                               \\
                            &                                                                                     & SEM                                                                   &                        & 89.82                     &                        & \multicolumn{1}{l}{89.67}          &                        & \multicolumn{1}{l}{\textbf{87.98}} &                        & \multicolumn{1}{l}{\textbf{84.87}}              &                        & \multicolumn{1}{l}{\textbf{18.78}}  \\ 
\midrule
\multirow{10}{*}{CIFAR-100} & \multirow{5}{*}{$2/255$}                                                            & EM                                                                     & \multirow{5}{*}{68.91} & 68.51                     & \multirow{5}{*}{66.54} & 68.72                              & \multirow{5}{*}{64.21} & 67.96                              & \multirow{5}{*}{58.35} & 68.44                                           & \multirow{5}{*}{47.99} & 68.49                               \\
                            &                                                                                     & TAP                                                                    &                        & \textbf{68.05}            &                        & 67.83                              &                        & 67.75                              &                        & 67.27                                           &                        & 66.91                               \\
                            &                                                                                     & Shortcut                                                                   &                        & 68.52                     &                        & 68.82                              &                        & 68.36                              &                        & 68.71                                           &                        & 66.53                               \\
                            &                                                                                     & REM                                                                    &                        & 69.00                     &                        & 68.20                              &                        & \textbf{60.75}                     &                        & \textbf{52.33}                                  &                        & 7.03                                \\
                            &                                                                                     & SEM                                                                   &                        & \multicolumn{1}{l}{68.59} &                        & \multicolumn{1}{l}{\textbf{66.79}} &                        & \multicolumn{1}{l}{61.44}          &                        & \multicolumn{1}{l}{52.56}                       &                        & \textbf{3.00}                       \\ 
\cmidrule{2-13}
                            & \multirow{5}{*}{$4/255$}                                                            & EM                                                                     & \multirow{5}{*}{64.50} & 63.86                     & \multirow{5}{*}{61.73} & 64.24                              & \multirow{5}{*}{57.61} & 63.62                              & \multirow{5}{*}{53.86} & 63.37                                           & \multirow{5}{*}{44.79} & 63.43                               \\
                            &                                                                                     & TAP                                                                    &                        & \textbf{63.21}            &                        & \textbf{63.01}                     &                        & \textbf{62.95}                     &                        & 62.90                                           &                        & 62.39                               \\
                            &                                                                                     & Shortcut                                                                   &                        & 63.48                     &                        & 63.59                              &                        & 63.64                              &                        & \textbf{62.83}                                  &                        & 62.44                               \\
                            &                                                                                     & REM                                                                    &                        & 63.75                     &                        & 63.99                              &                        & 64.36                              &                        & \begin{tabular}[c]{@{}c@{}}63.05\\\end{tabular} &                        & 27.10                               \\
                            &                                                                                     & SEM                                                                   &                        & 64.35                     &                        & 63.74                              &                        & 64.89                              &                        & 63.14                                           &                        & \textbf{20.08}                      \\
\hline
\end{tabular}
}

% \vspace{-3mm}
\label{tab: diff-ratio}
\end{table*}


==> tab/mmd.tex <==
\begin{table}[H]
\centering
\caption{Time costs for training different defensive noise generators on different datasets.}
\label{tab:mmd}
%\scriptsize
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c c c c c c c}
\toprule
Methods&Dataset & MMD value & p-value & Detect Successful Rate (DSR) & Detected?\\
\midrule
\multirow{3}{*}{Ours} &
CIFAR-10          &   &  & &  \\
&CIFAR-100          &   &  & &\\
&ImageNet  Subset   &   &  & &\\
\midrule
\multirow{3}{*}{Ours (adaptive)} &
CIFAR-10          &   &  & &  \\
&CIFAR-100          &   &  & &\\
&ImageNet  Subset   &   &  & &\\
\bottomrule
\end{tabular}
}
\end{table}


==> tab/noise_type.tex <==

\begin{table}
    \centering
    \caption{Effect of different types of random perturbation. The defensive noise radius is set to $8/255$.}
    \label{tab: diff_radius_random}
\resizebox{0.9\linewidth}{!}{
    \begin{tabular}{cccccc} 
        \toprule
        Dataset                    & Adv. Train. $\rho_a$ & \multicolumn{1}{c}{Zero}                                       & \multicolumn{1}{c}{Uniform} & \multicolumn{1}{c}{Gaussian} & \multicolumn{1}{c}{Beta}  \\ 
        \midrule
        \multirow{2}{*}{CIFAR-10} & $0$                  & 16.88  & 15.91 & 15.45 & \textbf{12.64 }    \\
        & $4/255$              & 35.78  & \textbf{29.33} & 36.54 & 31.92     \\ 
        \midrule
        \multirow{2}{*}{CIFAR-100}& $0$                  &  8.30 & 7.30   & 5.54  & \textbf{1.96}      \\
        & $4/255$              & 24.55  & \textbf{19.24} & 19.70 & 20.25     \\
        \bottomrule
        \end{tabular}
}
\end{table}

==> tab/trans.tex <==

\begin{table*}[htbp]
\centering
\label{tab:trans}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccccccccc} 
\toprule
\multirow{2}{*}{Dataset}         & \multirow{2}{*}{Source Model} & \multicolumn{5}{c}{REM} & \multicolumn{5}{c}{SEM}                                                          \\ 

                                 % &                               &             &                      \\
                     \cmidrule(l){3-7}
                     \cmidrule(l){8-12}
                                 &                               & VGG-16 & RN-18 & RN-50 & DN-121 & WRN-34-10 & VGG-16 & RN-18 & RN-50 & DN-121 & WRN-34-10  \\ 
\midrule
\multirow{5}{*}{CIFAR-10}        & VGG-16                        &        &       &       &        &           &        &       &       &        &            \\
                                 & RN-18                         &        &       &       &        &           &        &       &       &        &            \\
                                 & RN-50                         &        &       &       &        &           &        &       &       &        &            \\
                                 & DN-121                        &        &       &       &        &           &        &       &       &        &            \\
                                 & WRN-34-10                     &        &       &       &        &           &        &       &       &        &            \\ 
\midrule
\multirow{5}{*}{CIFAR-100}       & VGG-16                        &        &       &       &        &           &        &       &       &        &            \\
                                 & RN-18                         &        &       &       &        &           &        &       &       &        &            \\
                                 & RN-50                         &        &       &       &        &           &        &       &       &        &            \\
                                 & DN-121                        &        &       &       &        &           &        &       &       &        &            \\
                                 & WRN-34-10                     &        &       &       &        &           &        &       &       &        &            \\ 
\bottomrule
\end{tabular}

}
\caption{Test accuracy (\%) of different types of models on CIFAR-10 and CIFAR-100 datasets. The adversarial training perturbation radius is set as $4/255$. The defensive perturbation radius $\rho_u$ of every type of defensive noise is set as $8/255$.}
\end{table*}


==> tab/vis-cifar10.tex <==
%\subsection{}
\begin{figure*}[thbp]
% \centering
\addfigs{cifar10}{rad-8}{1250}{}{1.0}
\hspace{0.2cm}
\addfigs{cifar10}{rad-8}{1251}{}{1.0}
%\addfigs{cifar10}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
%\hspace{0.2cm}
%\addfigs{cifar10}{rad-16}{7}{Defensive perturbation radius $\rho_u = 16/255$.}
%\vspace{0.4cm}
%
%\addfigs{cifar10}{rad-8}{25344}{Defensive perturbation radius $\rho_u = 8/255$.}
%\hspace{0.2cm}
%\addfigs{cifar10}{rad-16}{25344}{Defensive perturbation radius $\rho_u = 16/255$.}
%\vspace{0.4cm}



%
%\addfigs{cifar10}{rad-8}{7}{Defensive perturbation radius $\rho_u = 8/255$.}
%\hspace{0.2cm}
%\addfigs{cifar10}{rad-16}{7}{Defensive perturbation radius $\rho_u = 16/255$.}
\addfigs{cifar10}{rad-8}{1252}{}{1.0}
\hspace{0.2cm}
% \vspace{0.4cm}
\addfigs{cifar10}{rad-8}{1253}{}{1.0}
%\addfigs{cifar10}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
%\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{5337}{ImageNet Subset}
\addfigs{cifar10}{rad-8}{1254}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar10}{rad-8}{1255}{}{1.0}
%\addfigs{cifar10}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{cifar10}{rad-8}{1256}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar10}{rad-8}{1257}{}{1.0}
%\addfigs{cifar10}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{cifar10}{rad-8}{1258}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar10}{rad-8}{1259}{}{1.0}
%\addfigs{cifar10}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{cifar10}{rad-8}{1260}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar10}{rad-8}{1261}{}{1.0}
%\addfigs{cifar10}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}

\addfigs{cifar10}{rad-8}{1262}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar10}{rad-8}{1263}{}{1.0}
%\addfigs{cifar10}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\caption{
More Visualization results on CIFAR-10. Examples of data are protected by error-minimizing noise (EM), targeted adversarial poisoning noise (TAP), shortcut noise (SC), robust error-minimizing noise (REM), and stable error-minimizing noise (SEM).
Note that $\rho_u$ is set as $8/255$ and the adversarial perturbation radius $\rho_a$ is set as $4/255$.
}
\label{fig:more-vis-example}
\end{figure*}

==> tab/vis-cifar100.tex <==
%\subsection{}{1.0}
\begin{figure*}[thbp]
% \centering
\addfigs{cifar100}{rad-8}{1264}{}{1.0}
\hspace{0.2cm}
\addfigs{cifar100}{rad-8}{1265}{}{1.0}
\vspace{0.4cm}

\addfigs{cifar100}{rad-8}{1266}{}{1.0}
\hspace{0.2cm}
% \vspace{0.4cm}
\addfigs{cifar100}{rad-8}{1253}{}{1.0}
%\addfigs{cifar100}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
%\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{5337}{ImageNet Subset}
\addfigs{cifar100}{rad-8}{1254}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar100}{rad-8}{1255}{}{1.0}
%\addfigs{cifar100}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{cifar100}{rad-8}{1256}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar100}{rad-8}{1257}{}{1.0}
%\addfigs{cifar100}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{cifar100}{rad-8}{1258}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar100}{rad-8}{1259}{}{1.0}
%\addfigs{cifar100}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{cifar100}{rad-8}{1260}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar100}{rad-8}{1261}{}{1.0}
%\addfigs{cifar100}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}

\addfigs{cifar100}{rad-8}{1262}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{ImageNet Subset}
\addfigs{cifar100}{rad-8}{1263}{}{1.0}
%\addfigs{cifar100}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\caption{
More Visualization results on CIFAR-100. Examples of data are protected by error-minimizing noise (EM), targeted adversarial poisoning noise (TAP), shortcut noise (SC), robust error-minimizing noise (REM), and stable error-minimizing noise (SEM).
Note that $\rho_u$ is set as $8/255$ and the adversarial perturbation radius $\rho_a$ is set as $4/255$.
}
\label{fig:more-vis-example-cifar100}
\end{figure*}

==> tab/vis-img-sub.tex <==
%\subsection{}{1.0}
\begin{figure*}[thbp]
% \centering
\addfigs{img-three}{rad-8}{1000}{}{1.0}
\hspace{0.2cm}
\addfigs{img-three}{rad-8}{1001}{}{1.0}
\vspace{0.4cm}

\addfigs{img-three}{rad-8}{1052}{}{1.0}
\hspace{0.2cm}
% \vspace{0.4cm}
\addfigs{img-three}{rad-8}{1152}{}{1.0}
%\addfigs{img-three}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
%\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{5337}{}{1.0}
\addfigs{img-three}{rad-8}{1223}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{}{1.0}
\addfigs{img-three}{rad-8}{1259}{}{1.0}
%\addfigs{img-three}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{img-three}{rad-8}{1305}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{}{1.0}
\addfigs{img-three}{rad-8}{1312}{}{1.0}
%\addfigs{img-three}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{img-three}{rad-8}{1348}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{}{1.0}
\addfigs{img-three}{rad-8}{1463}{}{1.0}
%\addfigs{img-three}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\addfigs{img-three}{rad-8}{1596}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{}{1.0}
\addfigs{img-three}{rad-8}{1676}{}{1.0}
%\addfigs{img-three}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}

\addfigs{img-three}{rad-8}{1929}{}{1.0}
\hspace{0.2cm}
% \addfigs{in-two}{rad-8}{12187}{}{1.0}
\addfigs{img-three}{rad-8}{1984}{}{1.0}
%\addfigs{img-three}{rad-16}{1}{Defensive perturbation radius $\rho_u = 16/255$.}
\vspace{0.4cm}
\caption{
More Visualization results on ImageNet Subset. Examples of data are protected by error-minimizing noise (EM), targeted adversarial poisoning noise (TAP), shortcut noise (SC), robust error-minimizing noise (REM), and stable error-minimizing noise (SEM).
Note that $\rho_u$ is set as $8/255$ and the adversarial perturbation radius $\rho_a$ is set as $4/255$.
}
\label{fig:more-vis-img-sub}
\end{figure*}
